MovieChat+: Question-aware Sparse Memory for Long Video Question Answering

Recently, integrating video foundation models and large language models to build a video understanding system can overcome the limitations of specific pre-defined vision tasks. Yet, existing methods either employ complex spatial-temporal modules or rely heavily on additional perception models to extract temporal features for video understanding, and they only perform well on short videos. For long videos, the computational complexity and memory costs associated with long-term temporal connections are significantly increased, posing additional challenges.Taking advantage of the Atkinson-Shiffrin memory model, with tokens in Transformers being employed as the carriers of memory in combination with our specially designed memory mechanism, we propose MovieChat to overcome these challenges. We lift pre-trained multi-modal large language models for understanding long videos without incorporating additional trainable temporal modules, employing a zero-shot approach. MovieChat achieves state-of-the-art performance in long video understanding, along with the released MovieChat-1K benchmark with 1K long video, 2K temporal grounding labels, and 14K manual annotations for validation of the effectiveness of our method. The code along with the dataset can be accessed via the following https://github.com/rese1f/MovieChat.

==> alg/Temp.tex <==
% \algnewcommand{\Comment}[1]{\textcolor{blue}{\(\triangleright\) #1}}
% \begin{algorithm}[t]
% \caption{Memory consolidation}\label{alg:alg}
% \begin{algorithmic}
% \Require $\mathcal{S}$ {\Comment{short-term memory}}
% \vspace{-10pt}
% \State \For{$\mathbf{x}_{i}$ in $\mathcal{S}$}
% \State \hspace{0.5cm} $s^{q} \gets sim(\mathbf{x}_{i}, \mathbf{q})$ \hfill\textcolor{global}{\(\triangleright\) question and frame similarity}
% \EndFor
% \vspace{-10pt}
% \State \If {\( \text{mean}(s^{q}) > \sigma \)} \hfill \textcolor{global}{\(\triangleright\) target merging threshold}
% \State \hspace{0.5cm} $M \gets M_0$
% \vspace{-10pt}
% \State \Else
% \State \hspace{0.5cm} $M \gets \alpha M_0$
% \EndIf
% \vspace{-10pt}
% \State \While{$len(\mathcal{S}) \textgreater M$} \hfill \textcolor{global}{\(\triangleright\) iterative merge}
% \vspace{-10pt}
% \State \For{$\mathbf{x}_{i}$ in $\mathcal{S}$}
% \State \hspace{0.5cm} $s^{f} \gets sim(\mathbf{x}_{i}, \mathbf{x}_{i+1})$ \hfill\textcolor{global}{\(\triangleright\)tokens similarity}
% \EndFor
% \State \hspace{0.25cm} $m \gets max(s^{f})$ \hfill\textcolor{global}{\(\triangleright\)the maximum value index}
% \State \hspace{0.25cm} $\mathbf{x}_{m} \gets merge (\mathbf{x}_{m},\mathbf{x}_{m+1})$ \hfill\textcolor{global}{\(\triangleright\)merge}
% \State \textbf{del} $\mathbf{x}_{m+1}$
% \EndWhile
% \label{alg}
% \end{algorithmic}
% \end{algorithm}

==> alg/longterm.tex <==
\definecolor{global}{RGB}{21,96,130}
\definecolor{breakpoint}{RGB}{51,0,111}

\begin{algorithm}[t]
\caption{Memory consolidation}\label{alg:longterm}
\begin{algorithmic}[1]
\Require $\mathcal{S}$ \textcolor{global}{\Comment{short-term memory}}
\While{$len(\mathcal{S}) \textgreater R_{L}$} \textcolor{global}{\Comment{iterative merge}}
\For{$\mathbf{x}_{i}$ in $\mathcal{S}$}
\State $s \gets sim(\mathbf{x}_{i}, \mathbf{x}_{i+1})$ \textcolor{global}{\Comment{tokens similarity}}
\EndFor
\State $m \gets max(s)$ \textcolor{global}{\Comment{the maximum value index}}
\State $\mathbf{x}_{m} \gets merge (\mathbf{x}_{m},\mathbf{x}_{m+1})$ \textcolor{global}{\Comment{merge}}
\State \textbf{del} $\mathbf{x}_{m+1}$
\EndWhile
\end{algorithmic}
\end{algorithm}


==> fig/ablation.tex <==
% \begin{figure*}[t]
%   \centering
%   \subfloat[\textbf{Category.}]
%   {
%       \includegraphics[width=0.32\textwidth]{fig/_category.pdf}
%   }
%   \subfloat[\textbf{Question type.}]
%   {
%       \includegraphics[width=0.32\textwidth]{fig/_questiontype.pdf}
%   }
%   \subfloat[\textbf{Video length.}]
%   {
%       \includegraphics[width=0.32\textwidth]{fig/_length.pdf}}
%   }
%   \centering
%   \caption{}
%   \label{fig:ablation_loss} 
% \end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{fig/_ablation.pdf}
  \caption{Hyperparameter ablation studies on how length of long-term memory buffer $l_{length}$, short-term memory buffer $l_{short}$, consolidation length $l_{merge}$ and short-term initialization affect the performance of MovieChat on long video understanding. We set $l_{short}=16$, $l_{merge}=2$ in ablation study of long-term memory,  $l_{long}=256$, $l_{merge}=2$ in ablation study of short-term memory and $l_{short}=16$ in ablation study of consolidation length and short-term initialization. }
  \label{fig:ablation}
\end{figure*}

% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}{\textwidth}
%     \centering
%     \includegraphics[width=0.25\textwidth]{fig/_long_abl.pdf}
%     \label{fig:long_abl}
%   \end{subfigure}
%   \begin{subfigure}{\textwidth}
%     \centering
%     \includegraphics[width=0.25\textwidth]{fig/_short_abl.pdf}
%     \label{fig:short_abl}
%   \end{subfigure}
%   \begin{subfigure}{\textwidth}
%     \centering
%     \includegraphics[width=0.25\textwidth]{fig/_initial_abl.pdf}
%     \label{fig:initial_abl}
%   \end{subfigure}
%   \caption{Hyperparameter ablation studies on how length of long-term memory buffer $l_{length}$, short-term memory buffer $l_{short}$, consolidation length $l_{merge}$ and short-term initialization affect the performance of MovieChat on long video understanding. We set $l_{short}=16$, $l_{merge}=2$ in ablation study of long-term memory,  $l_{long}=2^{8}$, $l_{merge}=2$ in ablation study of short-term memory and $l_{short}=16$ in ablation study of consolidation length and short-term initialization. }
%   \label{fig:ablation}
% \end{figure*}



==> fig/answer.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=1\linewidth]{fig/_total_answer.pdf}
    \vspace{-45pt}
    \caption{Length of total answers.}
    \label{fig:subfig-a}
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \vspace{-30pt}
    \includegraphics[width=1\linewidth]{fig/_global_answer.pdf}
    \vspace{-45pt}
    \caption{Length of global answers.}
    \label{fig:subfig-b}
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \vspace{-30pt}
    \includegraphics[width=1\linewidth]{fig/_break_answer.pdf}
    \vspace{-45pt}
    \caption{Length of breakpoint answers.}
    \label{fig:subfig-c}
  \end{subfigure}
  \caption{Length distribution of answers.}
  \label{fig:answer}
\end{figure}



==> fig/benchmark.tex <==
\begin{figure*}[t]
  \centering

  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_category3.pdf}
    \caption{\textbf{Category.}}
    \label{fig:category}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_length.pdf}
    \caption{\textbf{Video length.}}
    \label{fig:video_length}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_questiontype.pdf}
    \caption{\textbf{Question type.}}
    \label{fig:question_type}
  \end{subfigure}
  \caption{Video-text statistics in MovieChat-1K. It encompasses a diverse set of categories, gathered from multiple question types and containing a diverse distribution of clip durations. We annotate the video categories that account for more than 4.5\% of the total (the complete list of video categories and their percentages in Appendix). ``frm" represents the number of video frames.}
  \label{fig:benchmark}
\end{figure*}



==> fig/case2.tex <==
\begin{figure*}[!t]
	\centering
    \includegraphics[width=0.95\linewidth]{fig/_case_3.pdf}
	\caption{Question and answer about clips from \textit{Game of Thrones}, which tells the epic fantasy tale of power struggles and political intrigue among the Seven Kingdoms, entwined with intricate family relationships, all set against the backdrop of an ancient, mystical threat.}
    \label{fig:case3}
    \vspace{20pt}
    \includegraphics[width=0.95\linewidth]{fig/_case_4.pdf}
	\caption{Question and answer about clips from \textit{YouTube}, which contains a compilation of some inspirational movies scenes. This video clip comprises several segments from \textit{The Death Crawl}, \textit{Coach Carter}, \textit{Rocky Balboa}, and \textit{We Are Marshall}, which vary in duration.}
    \label{fig:case4}
 \vspace{20pt}

\end{figure*}

==> fig/case_tpami.tex <==
\begin{figure*}[!t]
	\centering
    \includegraphics[width=0.95\linewidth]{fig/_case_1.pdf}
	\caption{Question and answer about clips from \textit{Zootopia}, a cartoon, which tells the story of a determined police officer rabbit named Judy who pairs up with a cunning fox to uncover a conspiracy about missing animals and develop an unexpected friendship.}
        \label{fig:case1}
    \vspace{20pt}
    \includegraphics[width=0.95\linewidth]{fig/_case_2.pdf}
	\caption{Question and answer about clips from \textit{Goblin}, which tells the story of Kim Shin, an immortal "goblin" who needs to find a human bride to end his endless life but instead meets Ji Eun-tak, a girl fated to die who claims to be the "goblin's bride," leading to a romantic tale unfolding between them.}
        \label{fig:case2}
 \vspace{20pt}
\end{figure*}

==> fig/category.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/_category.pdf}
    \caption{\textbf{Category.}}
    \label{fig:category}
\end{figure}

==> fig/certi.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.88\linewidth]{fig/_certi.pdf}
    \vspace{-12pt}
    \captionsetup{font={scriptsize}}
    \caption{Certificate length across video datasets.}
    \label{fig:certi}
\end{figure}


% \begin{figure}[ht]
%     \begin{minipage}{0.5\linewidth}
%         \centering        \includegraphics[width=\linewidth]{fig/_certi.pdf}
%         \vspace{-22pt}
%         \caption{ }
%         \label{fig:certi}
%     \end{minipage}%
%     \begin{minipage}{0.5\linewidth}
%         \centering        \includegraphics[width=\linewidth]{fig/_reb_abl.pdf}
%         \vspace{-22pt}
%         \caption{ }
%         \label{fig:reb_abl}
%     \end{minipage}
% \end{figure}



==> fig/data_format.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{fig/_data_format.pdf}
    \caption{Video information and visual question-answer data format in MovieChat1K. }
    \label{fig:data_format}
\end{figure*}

==> fig/intro.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/_intro.pdf}
    \caption{VRAM cost under gigabyte (GB) (y-axis) v.s. frame number (x-axis) comparison. We test the visual-only inference of all methods at a resolution of $224 \times 224$ without frame sampling. While the previous method can only support around $100$ frames of inference, MovieChat can handle videos with $\textgreater 10$K frames on a 24GB graphics card. MovieChat has a $10000 \times$ advantage over other methods in terms of the average increase in VRAM cost per frame ($21.3$KB to $\sim200$MB per frame).}
    \label{fig:intro}
\end{figure}

==> fig/length.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/_length.pdf}
    \caption{\textbf{Average clip length.}}
    \label{fig:length}
\end{figure}

==> fig/llm.tex <==
\definecolor{global}{RGB}{21,96,130}
\definecolor{breakpoint}{RGB}{51,0,111}
\definecolor{hall}{RGB}{183,165,122}

\begin{figure*}[!t]
	\centering
    \includegraphics[width=0.95\linewidth]{fig/_llm2.pdf}
	\caption{Question and answer about clips from \textit{YouTube}, which is a tutorial on how to cook steak. When asked ``Which step took the longest to complete this dish?" in global mode, MovieChat powered by different large language models provided divergent answers.}
 \vspace{20pt}
\label{fig:llm}
\end{figure*}



==> fig/merge.tex <==
\definecolor{global}{RGB}{21,96,130}
\definecolor{breakpoint}{RGB}{51,0,111}
\definecolor{hall}{RGB}{183,165,122}

\begin{figure*}[!t]
	\centering
    \includegraphics[width=0.8\linewidth]{fig/_merge.pdf}
	\caption{Question and answer about clips from \textit{YouTube}, which is a tutorial on how to cook steak. The entire instructional process begins with marinating the steak, followed by pan-searing it, preparing side dishes, and ultimately plating the meal.}
 \vspace{20pt}
\label{fig:merge}
\end{figure*}



==> fig/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.84\linewidth]{fig/_overview.pdf}
    \caption{\textbf{Illustration of MovieChat.} MovieChat extracts video features with a sliding window and represents them in token form, which are then sequentially fed into the short-term memory frame by frame. When the fixed-length short-term memory reaches its preset limit, the earliest tokens are popped and consolidated into the long-term memory. MovieChat incorporates two distinct inference modes: the global mode, which exclusively utilizes the long-term memory, and the breakpoint mode, which additionally incorporates the current short-term memory as part of the video representation. The breakpoint mode allows for understanding the video at a specific moment in time. After passing through a projection layer, the video representation is inputted into a large language model for interaction with the user.}
    \label{fig:overview}
\end{figure*}

% We use a sliding window approach to extract video features and represent them in token form, which are then sequentially fed into the short-term memory frame by frame. The short-term memory has a fixed length, and when it reaches its set limit, the earliest tokens are popped and consolidated into the long-term memory. We have designed two inference modes: global mode, which exclusively utilizes the long-term memory, and breakpoint mode, which additionally incorporates the current short-term memory as part of the video representation. Breakpoint mode allows for understanding the video at a specific moment in time. Finally, after passing through a projection layer, the video representation is inputted into a large language model for interaction with the user.





==> fig/pear.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_gpt-claude.pdf}
    \caption{\textbf{GPT-3.5 VS. Claude} \\ \centering PCC = 0.927}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_gpt-human.pdf}
    \caption{\textbf{GPT-3.5 VS. Human Blind Rating} \\ \centering PCC = 0.955}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/_human-claude.pdf}
    \caption{\textbf{Claude VS. Human Blind Rating} \\ \centering PCC = 0.978}
  \end{subfigure}
  \caption{Results of the Pearson correlation analysis between three evaluation methods, including GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage}, and human blind rating. PCC stands for Pearson Correlation Coefficient.}
  \label{fig:pearson}
\end{figure*}

==> fig/prompt.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{fig/_prompt.pdf}
    \caption{Prompt for ChatGPT in LLM-Assisted Evaluation for the short video question-answering task.}
    \label{fig:prompt}
\end{figure*}

==> fig/question.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=1\linewidth]{fig/_total_question.pdf}
    \vspace{-45pt}
    \caption{Length of total questions.}
    \label{fig:subfig-a}
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \vspace{-30pt}
    \includegraphics[width=1\linewidth]{fig/_global_question.pdf}
    \vspace{-45pt}
    \caption{Length of global questions.}
    \label{fig:subfig-b}
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \vspace{-30pt}
    \includegraphics[width=1\linewidth]{fig/_break_question.pdf}
    \vspace{-45pt}
    \caption{Length of breakpoint questions.}
    \label{fig:subfig-c}
  \end{subfigure}
  \caption{Length distribution of questions.}
  \label{fig:question}
\end{figure}



==> fig/questiontype.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/_questiontype.pdf}
    \caption{\textbf{Question type.}}
    \label{fig:questiontype}
\end{figure}

==> fig/rebuttal_abl.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/_reb_abl.pdf}
    \caption{Replotting of Figure 5.}
    \label{fig:reb_abl}
\end{figure}

==> tab/Pearson.tex <==
\begin{table}[h]
\centering
\Large
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ l | c }
\toprule
Evaluation Method & Pearson Correlation Coefficient\\
\midrule

GPT3.5 VS. Claude & 0.927\\
GPT3.5 VS. Human Blind Rating & 0.955\\
Claude VS. Human Blind Rating & 0.978\\
\bottomrule
\end{tabular}
}
\caption{Pearson correlation coefficient of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage}, and human blind rating on score. We calculate the mean score across each score dimensions for MovieChat and previous methods~\cite{maaz2023video,li2023videochat,zhang2023llama, zhang2023video}, and then computes the Pearson correlation between these means for each pair of evaluation methods. The Pearson correlation coefficient, which ranges from -1 to +1, indicates a stronger positive linear relationship between the two sets of data when the coefficient is higher (closer to +1).}
\label{tab:pearson}
\end{table}

==> tab/benchmarks.tex <==
\begin{table*}

\centering
\Large
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ c | c | c | c | c | c | c}
\toprule
Dataset & Avg. Duration (min) & Number of Captions & Avg. Caption Length & Number of Question-Answer Pairs & Avg. Question Length& Avg. Answer Length \\

\midrule
MovieQA~\cite{tapaswi2016movieqa} & 3.5 & - & - & 14.9K& 9.3& 5.1\\
MovieGraphs~\cite{vicol2018moviegraphs} & 0.73 & 15K& 35& - & - & -\\
MovieNet~\cite{huang2020movienet} & 2.1 & 2.5K & - & - & - & - \\
\midrule
MovieChat-1K & 9.4 & 1K & 121 & 13K& 7.8& 2.3\\
\bottomrule
\end{tabular}
}

\caption{Comparison between MovieChat-1K and other benchmarks.}
\label{tab:benchmarks}    
\end{table*}

==> tab/break_5.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 2.42 & \scriptsize 2.51 & \scriptsize 2.81 & \scriptsize 2.10 & \scriptsize 2.78\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.04 & \scriptsize 2.29& \scriptsize 2.63& \scriptsize 2.00& \scriptsize 2.87\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize \underline{2.62}& \scriptsize \textbf{2.65}& \scriptsize \underline{2.86}& \scriptsize \underline{2.32}& \scriptsize \underline{2.96}\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{2.64}& \scriptsize \underline{2.60}& \scriptsize \textbf{2.87}& \scriptsize \textbf{2.49}& \scriptsize \textbf{3.08} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in breakpoint mode with the average of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage} and human blind rating. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:break_5}
\end{table}


				

==> tab/break_5_claude.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 2.12 & \scriptsize 2.20 & \scriptsize 2.30& \scriptsize 1.97 & \scriptsize 2.37\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 1.62 & \scriptsize 1.85& \scriptsize 2.20& \scriptsize 1.34& \scriptsize 2.02\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize \underline{2.36}& \scriptsize \textbf{2.26}& \scriptsize \underline{2.34}& \scriptsize \underline{2.23}& \scriptsize \textbf{2.70}\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{2.38} & \scriptsize \underline{2.16}& \scriptsize \textbf{2.35}& \scriptsize \textbf{2.43}& \scriptsize \underline{2.68} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in breakpoint mode with Claude~\cite{examplewebpage}. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:break_5_claude}
\end{table}


				

==> tab/break_5_gpt.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 2.96 & \scriptsize 3.09 & \scriptsize 3.24& \scriptsize 2.46 & \scriptsize 3.22\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.42 & \scriptsize 2.85& \scriptsize 2.87& \scriptsize 2.00& \scriptsize 2.87\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize \textbf{3.11}& \scriptsize \textbf{3.32}& \scriptsize \underline{3.29}& \scriptsize \underline{2.62}& \scriptsize \underline{3.29}\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \underline{3.07}& \scriptsize \underline{3.24}& \scriptsize \textbf{3.31}& \scriptsize \textbf{2.70}& \scriptsize \textbf{3.45} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in breakpoint mode with GPT-3.5~\cite{gpt3.5}. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:break_5_gpt}
\end{table}


				

==> tab/break_5_human.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 2.17 & \scriptsize 2.24 & \scriptsize 2.89& \scriptsize 1.87 & \scriptsize 2.75\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.09 & \scriptsize 2.18& \scriptsize 2.82 & \scriptsize 1.74& \scriptsize 2.68\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize \underline{2.39}& \scriptsize \underline{2.36}& \scriptsize \textbf{2.96}& \scriptsize \underline{2.10}& \scriptsize \underline{2.89}\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{2.48}& \scriptsize \textbf{2.41}& \scriptsize \underline{2.94}& \scriptsize \textbf{2.33}& \scriptsize \textbf{3.12} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in breakpoint mode with human blind rating. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:break_5_human}
\end{table}


				

==> tab/cate.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{ c | c}
\toprule
\textbf{\tiny Category} & \textbf{\tiny Percentage} \\
\midrule
\tiny Documentary Film & \tiny 21.80\% \\
\tiny Animation Film & \tiny 17.00\% \\
\tiny Detective Film & \tiny 15.10\% \\
\tiny Epic Film & \tiny 11.40\% \\
\tiny Action Film & \tiny 6.70\% \\
\tiny Family Film & \tiny 4.90\% \\
\tiny Crime Film & \tiny 3.80\% \\
\tiny Science Fiction Film & \tiny 3.70\% \\
\tiny War Film & \tiny 3.70\% \\
\tiny Adventure Film & \tiny 3.50\% \\
\tiny Romance Film & \tiny 3.30\% \\
\tiny History Film & \tiny 2.10\% \\
\tiny Suspense Film & \tiny 1.30\% \\
\tiny Fantasy & \tiny 0.90\% \\
\tiny School Film & \tiny 0.80\% \\
\bottomrule
\end{tabular}
}
\caption{Distribution of video categories in MovieChat-1K.}
\label{tab:cate}
\end{table}

==> tab/class.tex <==
\begin{table}[h]
\centering
\tiny 
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.4}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c @{}}
\toprule
 \\[-2ex]
% \hspace{1cm} \tiny \textbf{Model}\hspace{1cm} & \tiny \textbf{Text Encoder} & \tiny \hspace{1cm} \textbf{VC Acc} \hspace{1cm} \\
\tiny \textbf{Model} & \tiny \textbf{Text Decoder} & \tiny \textbf{VC Acc} \\
 \\[-2ex]
\midrule
 \\[-2ex]
\multicolumn{2}{c}{\tiny Choosing the correct answer uniformly at random} & \tiny 14.3\% \\
 \\[-2ex]
\midrule
 \\[-2ex]
\tiny GIT & \tiny non-LLM based &  \tiny 22.6\% \\
\tiny mPLUG-2 & \tiny non-LLM based & \tiny 25.3\%  \\
\tiny Video Chat & \tiny LLM based & \tiny \underline{35.6\%} \\
 \\[-2ex]
\midrule
 \\[-2ex]
\textbf{\tiny MovieChat}& \tiny LLM based & \tiny \textbf{36.4\%}  \\
 \\[-1.5ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Classification evaluation on MovieChat-1K. }
\label{tab:class}
\end{table}

% sci fic -> Science fiction film, detective film, Adventure Film
% cartoon -> Animation Film
% thriller -> Crime Film, action film
% drama -> epic film
% 去除movie， television后人工筛选

==> tab/ego.tex <==
\begin{table}[h]
\centering
\tiny
\setlength{\tabcolsep}{8pt}
\setcellgapes{0.1pt} 
\makegapedcells
\renewcommand{\arraystretch}{0.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c @{}}
\toprule
 \\[-2ex]
% \hspace{1cm}\tiny \textbf{Model}\hspace{0.2cm}
%  & \hspace{2cm}\tiny \textbf{Text Encoder} \hspace{2cm} & \tiny \textbf{QA Acc} \hspace{3cm}\\
\tiny \textbf{Model}
 & \tiny \textbf{Text Decoder}  & \tiny \textbf{QA Acc}\\
 \\[-2ex]
\midrule
\\[-2ex]
\multicolumn{2}{c}{\tiny Choosing the correct answer uniformly at random} & \tiny  20.0\% \\
 \\[-2ex]
\midrule
 \\[-2ex]
% FrozenBiLM & non-LLM based & 26.9\% \\
% VIOLET  & non-LLM based & 19.9\% \\
% mPLUG-Owl & LLM based & 31.1\% \\
\tiny InternVideo& \tiny non-LLM based & \tiny 32.1\% \\
\tiny Video Chat & \tiny LLM based & \tiny 47.5\% \\
\tiny \textbf{MovieChat}  & \tiny LLM based & \tiny \underline{53.5\%} \\
 \\[-2ex]
\midrule
 \\[-2.5ex]
\multicolumn{2}{c}{\tiny Human Performance} & \tiny \textbf{76.2\%} \\
 \\[-2ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Zero-shot QA Evaluation on EgoSchema.}
\label{tab:ego}
\end{table}

==> tab/hyper-param.tex <==
\begin{table}[h]
\centering
\Large
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ c | c}
\toprule
Description & Default Value \\
\midrule
% $\alpha_{1}$ & 0.5 \\
% $\alpha_{2}$ & 0.5 \\
size of sliding window & $16$ frames\\
size of short-term memory & $18$ frames $\times$ $32$ tokens per frames\\
size of long-term memory & $256$ frames\\
consolidation length & 2 \\
\bottomrule
\end{tabular}
}
\caption{Hyper-parameter settings of MovieChat.}
\label{tab:hyper}
\end{table}

==> tab/llm_5.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Global Mode}} & \multicolumn{5}{c}{\textbf{Breakpoint Mode}} \\
\cline{2-11}
& \textbf{CI} & \textbf{DO} & \textbf{CU} & \textbf{TU} & \textbf{CO} & \textbf{CI} & \textbf{DO} & \textbf{CU} & \textbf{TU} & \textbf{CO}\\
\midrule
\midrule
LLama~\cite{touvron2023llama}&  \textbf{3.32}&  \textbf{3.28}&  3.40&  \textbf{2.97}& \textbf{3.48}& \textbf{2.97}& \textbf{3.24}& 3.31& \textbf{2.70}& 3.45 \\
LLama2~\cite{touvron2023llama2}&  3.27&  \textbf{3.28}&  \textbf{3.41} &  2.95& 3.45 & 2.96& 3.12& \textbf{3.38}& 2.68& \textbf{3.34}\\
\bottomrule
\end{tabular}
}
\caption{Ablation Study on how the large language model affects the long video generative performance. MM stands for memory mechanism, CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency.The best result is highlighted in bold.}
\label{tab:llm_5}
\end{table}



==> tab/llm_score.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{9pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c @{}}
\toprule
\multirow{2}{*}{\vspace{-0.5ex} \tiny \textbf{Method}} & \multicolumn{2}{c}{\tiny \textbf{Global Mode}} & \multicolumn{2}{c}{\tiny \textbf{Breakpoint Mode}} \\
\cline{2-5}
 & \tiny \textbf{Accuracy} & \tiny \textbf{Score} & \tiny \textbf{Accuracy} & \tiny \textbf{Score}\\
\midrule
\vspace{-0.5ex} \tiny LLama~\cite{touvron2023llama} & \tiny \textbf{67.8}& \tiny \textbf{3.81}& \tiny \textbf{50.4}& \tiny 2.96 \\
\vspace{-0.5ex} \tiny LLama2~\cite{touvron2023llama2}& \tiny 64.2& \tiny 3.79& \tiny 48.1& \tiny \textbf{2.98} \\
\bottomrule
\end{tabular}
}
\caption{Ablation Study on how LLM affects the long video question answering. The best result is highlighted in bold.}
\label{tab:llm_score}
\end{table}

==> tab/long.tex <==
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{} l c c c c c @{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
% \cline{3-6}
%  & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
% \midrule
% Video Chat~\cite{li2023videochat}& 32 & \underline{61.0} & \underline{3.34} & 48.3 & 2.43 \\
% Video LLaMA~\cite{zhang2023video}& 32 & 51.4 & 3.10 & 38.2 & 2.31 \\
% Video-ChatGPT~\cite{maaz2023video}& 100 & 44.2 & 2.71 & \underline{49.8} & \underline{2.71} \\ 
% \midrule
% MovieChat~\textit{(ours)} & 2048 & \textbf{67.8} & \textbf{3.81} & \textbf{50.4} & \textbf{2.96}\\
% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with GPT. The best result is highlighted in bold, and the second best is underlined.}
% \label{tab:long}
% \end{table}

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{} l c c c c c @{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
% \cline{3-6}
%  & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
% \midrule
% Video Chat~\cite{li2023videochat}& 32 & \underline{61.0/52.1/60.2} & \underline{3.34/2.59/3.08} & 48.3/43.8/46.3 & 2.43/2.12/2.32 \\
% Video LLaMA~\cite{zhang2023video}& 32 & 51.4/47.3/56.3 & 3.10/2.19/2.72 & 38.2/33.2/45.8 & 2.31/1.69/2.11 \\
% Video-ChatGPT~\cite{maaz2023video}& 100 & 44.2/39.8/58.7 & 2.71/2.04/2.89 & \underline{49.8/46.4/47.8} & \underline{2.71/2.21/2.43} \\ 
% \midrule
% MovieChat~\textit{(ours)} & 2048 & \textbf{67.8/55.3/63.7} & \textbf{3.81/2.73/3.15} & \textbf{50.4/46.4/48.1} & \textbf{2.96/2.28/2.46}\\
% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with GPT, Claude and human bling rating. The best result is highlighted in bold, and the second best is underlined.}
% \label{tab:long}
% \end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
\cline{3-6}
 & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\midrule
Video Chat~\cite{li2023videochat}& 32 & \underline{57.8} & \underline{3.00} & 46.1 & 2.29 \\
Video LLaMA~\cite{zhang2023video}& 32 & 51.7 & 2.67 & 39.1 & 2.04 \\
Video-ChatGPT~\cite{maaz2023video}& 100 & 47.6 & 2.55 & \underline{48.0} & \underline{2.45} \\ 
\midrule
MovieChat~\textit{(ours)} & 2048 & \textbf{62.3} & \textbf{3.23} & \textbf{48.3} & \textbf{2.57}\\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video question answering on MovieChat-1K test set in global mode with the average of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage} and human bling rating. HBR stands for human blind rating. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long}
\end{table}

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{} l c c c c c @{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
% \cline{3-6}
%  & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
% \midrule

% MovieChat~\textit{(ours)} & 2048 & \textbf{55.1} & \textbf{2.78} & \textbf{38.5} & \textbf{1.87}\\
% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with Gemini-Pro. We use Gemini-Pro for LLM-assisted evaluation in this challenge.}
% \label{tab:long}
% \end{table}

==> tab/long_claude.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
\cline{3-6}
 & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\midrule
Video Chat~\cite{li2023videochat}& 32 & \underline{52.1} & \underline{2.59} &  \underline{43.8}& 2.12 \\
Video LLaMA~\cite{zhang2023video}& 32 &  47.3& 2.19 & 33.2 & 1.69 \\
Video-ChatGPT~\cite{maaz2023video}& 100 & 39.8 & 2.04 & \textbf{46.4} & \underline{2.21} \\ 
\midrule
MovieChat~\textit{(ours)} & 2048 & \textbf{55.3}&  \textbf{2.73}&  \textbf{46.4}& \textbf{2.28}\\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with Claude~\cite{examplewebpage}. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_claude}
\end{table}

==> tab/long_gpt.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
\cline{3-6}
 & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\midrule
Video Chat~\cite{li2023videochat}& 32 & \underline{61.0} & \underline{3.34} & 48.3 & 2.43 \\
Video LLaMA~\cite{zhang2023video}& 32 & 51.4 & 3.10 & 38.2 & 2.31 \\
Video-ChatGPT~\cite{maaz2023video}& 100 & 44.2 & 2.71 & \underline{49.8} & \underline{2.71} \\ 
\midrule
MovieChat~\textit{(ours)} & 2048 & \textbf{67.8} & \textbf{3.81} & \textbf{50.4} & \textbf{2.96}\\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with GPT-3.5~\cite{gpt3.5}. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_gpt}
\end{table}

==> tab/long_human.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
\cline{3-6}
 & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\midrule
Video Chat~\cite{li2023videochat}& 32 & \underline{60.2} & \underline{3.08} &  46.3& 2.32 \\
Video LLaMA~\cite{zhang2023video}& 32 &  56.3& 2.72 & 45.8 & 2.11 \\
Video-ChatGPT~\cite{maaz2023video}& 100 & 58.7 & 2.89 & \underline{47.8} & \underline{2.43} \\ 
\midrule
MovieChat~\textit{(ours)} & 2048 & \textbf{63.7}&  \textbf{3.15}&  \textbf{48.1}& \textbf{2.46}\\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video question answering on MovieChat-1K test set with human blind rating. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_human}
\end{table}

==> tab/long_varies.tex <==
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{0.7}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{} l c c c c c c @{}}
% \toprule
% \scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
% \midrule
% \scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 3.26 & \scriptsize \underline{3.20} & \scriptsize \underline{3.38} & \scriptsize \underline{2.97}& \scriptsize  \underline{3.47}\\
% \scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize \underline{3.30} & \scriptsize 2.53& \scriptsize 3.28& \scriptsize 2.77& \scriptsize 3.42\\
% \scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize 2.48& \scriptsize 2.78& \scriptsize 3.03& \scriptsize 2.48& \scriptsize 2.99\\
% \midrule
% \scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{3.32}& \scriptsize \textbf{3.28} & \scriptsize \textbf{3.40}& \scriptsize \textbf{3.01}& \scriptsize \textbf{3.48} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative evaluation for long video generation performance in global mode with GPT. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
% \label{tab:long_varies}
% \end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.61}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize \underline{3.04} & \scriptsize \underline{2.75} & \scriptsize \underline{3.09} & \scriptsize \underline{3.00}& \scriptsize  \underline{3.21}\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.75 & \scriptsize 2.24& \scriptsize 2.83& \scriptsize 2.62& \scriptsize 2.97\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize 2.37& \scriptsize 2.30& \scriptsize 2.58& \scriptsize 2.49& \scriptsize 2.69\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{3.11}& \scriptsize \textbf{2.93} & \scriptsize \textbf{3.24}& \scriptsize \textbf{3.17}& \scriptsize \textbf{3.25} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in global mode with the average of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage} and human blind rating. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is in bold, and the second best is underlined.}
\label{tab:long_varies}
\end{table}

==> tab/long_varies_claude.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize \underline{2.83} & \scriptsize \underline{2.43} & \scriptsize \underline{3.02} & \scriptsize \underline{2.87}& \scriptsize  \underline{2.93}\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.04 & \scriptsize 1.66& \scriptsize 2.46& \scriptsize 2.07& \scriptsize 2.36\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize 1.81& \scriptsize 1.65& \scriptsize 2.05& \scriptsize2.07& \scriptsize 2.07\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{2.88}& \scriptsize \textbf{2.82} & \scriptsize \textbf{3.11}& \scriptsize \textbf{3.04}& \scriptsize \textbf{2.96} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in global mode with Claude~\cite{examplewebpage}. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_varies_claude}
\end{table}

==> tab/long_varies_gpt.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize 3.26 & \scriptsize \underline{3.20} & \scriptsize \underline{3.38} & \scriptsize \underline{2.97}& \scriptsize  \underline{3.47}\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize \underline{3.30} & \scriptsize 2.53& \scriptsize 3.28& \scriptsize 2.77& \scriptsize 3.42\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize 2.48& \scriptsize 2.78& \scriptsize 3.03& \scriptsize 2.48& \scriptsize 2.99\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{3.32}& \scriptsize \textbf{3.28} & \scriptsize \textbf{3.44}& \scriptsize \textbf{3.06}& \scriptsize \textbf{3.48} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in global mode with GPT-3.5~\cite{gpt3.5}. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_varies_gpt}
\end{table}


==> tab/long_varies_human.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize \underline{3.03} & \scriptsize \underline{2.61} & \scriptsize \underline{2.87} & \scriptsize \underline{3.15}& \scriptsize  \underline{3.23}\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 2.91 & \scriptsize 2.54& \scriptsize 2.74& \scriptsize 3.01& \scriptsize 3.12\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize 2.83& \scriptsize 2.47& \scriptsize 2.66& \scriptsize2.92& \scriptsize 3.01\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{3.12}& \scriptsize \textbf{2.68} & \scriptsize \textbf{3.17}& \scriptsize \textbf{3.41}& \scriptsize \textbf{3.31} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for long video generation performance in global mode with human blind rating. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:long_varies_claude}
\end{table}

==> tab/mplug-acc.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c | c c c c @{}}
\toprule
% \multirow{}{}{\textbf{Method}} & \multirow{}{}{\textbf{\# Frames}} & \multicolumn{2}{c}{\textbf{Global Mode}} & \multicolumn{2}{c}{\textbf{Breakpoint Mode}} \\
% \cline{3-6}
%  & & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} \\
\textbf{Method} & \textbf{Frames} & \textbf{Global Acc} & \textbf{Global Score} & \textbf{Breakpoint Acc} & \textbf{Breakpoint Score} \\
\midrule
\scriptsize GIT & 6 & 28.8 & 1.83 & 29.2 & 1.98 \\
\scriptsize mPLUG-2 & \scriptsize 8 & \scriptsize 31.7 & \scriptsize 2.13 & \scriptsize 30.8 & \scriptsize 1.83 \\
\scriptsize Video Chat& 32 & \underline{51.7} & \underline{2.67} & \underline{39.1} & \underline{2.04} \\
\midrule
\textbf{MovieChat~\textit{(ours)}} & 2048 & \textbf{62.3} & \textbf{3.23} & \textbf{48.3} & \textbf{2.57}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Long video QA evaluation on MovieChat-1K test set.}
\label{tab:mplug-acc}
\end{table}

==> tab/mplug-short.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c | c c @{}}
\toprule

\textbf{Method} & \textbf{Text Decoder} & \hspace{0.3cm}\textbf{MSVD-QA}\hspace{0.3cm} & \hspace{0.3cm}\textbf{MSRVTT-QA}\hspace{0.3cm} \\
\midrule

VideoCoCa & non-LLM based & 56.9 & 46.0 \\

GIT & non-LLM based & 56.8 & 43.2 \\

 mPLUG-2 &  non-LLM based &  58.1 &  48.0 \\
 
 % \rowcolor{purple!5}
 Video-ChatGPT &  LLM based &  \underline{64.9} &  \underline{49.3}\\ 
\midrule
\textbf{ MovieChat~\textit{(Ours)}} &  LLM based &  \textbf{75.2} & \textbf{52.7}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Evaluation for short video question answering.}
\label{tab:mplug-short}
\end{table}

==> tab/mplug_5.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.61}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c | c c c c c c @{}}
\toprule
 \\[-2ex]
\hspace{0.5cm}\scriptsize \textbf{Method} \hspace{0.5cm} & \hspace{0.1cm} \scriptsize \textbf{CI} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{DO}\hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{CU} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{TU} \hspace{0.1cm} & \hspace{0.1cm} \scriptsize \textbf{CO} \hspace{0.5cm}\\
 \\[-2ex]
\midrule
 \\[-2ex]
\scriptsize GIT & \scriptsize 1.65  & \scriptsize 1.74  & \scriptsize 2.00  & \scriptsize 1.88  & \scriptsize 2.16 \\
\scriptsize mPLUG-2 & \scriptsize 1.82 & \scriptsize 1.93 & \scriptsize 2.24 & \scriptsize 1.92 & \scriptsize 2.35\\
\scriptsize Video Chat & \scriptsize \underline{3.04} & \scriptsize \underline{2.75} & \scriptsize \underline{3.09} & \scriptsize \underline{3.00}& \scriptsize  \underline{3.21}\\
 \\[-1.7ex]
\midrule
 \\[-1.8ex]
\hspace{0.3cm} \textbf{\scriptsize MovieChat~\textit{(Ours)}} \hspace{0.1cm}& \scriptsize \textbf{3.11}& \scriptsize \textbf{2.93} & \scriptsize \textbf{3.24}& \scriptsize \textbf{3.17}& \scriptsize \textbf{3.25} \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Long video QA results on MovieChat-1K in global mode.}
\label{tab:mplug-5}
\end{table}

==> tab/question_type.tex <==
\begin{table}[h]
\centering
\tiny
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c | c c | c c @{}}
\toprule
 \\[-2ex]
\tiny \textbf{Type} & \tiny \textbf{Rate} & \tiny \textbf{Frame Type}& \tiny \textbf{Text Rate} & \tiny \textbf{Type} & \tiny \textbf{Text Rate}\\
 \\[-2ex]
\midrule
 \\[-2ex]
    Location & 21.2\% & Scene & 11.2\% & Existence & 5.0\% \\

    Time & 17.2\% & Object & 10.7\% & Weather & 3.6\% \\

    Number & 14.6\% & Action & 7.8\% & Others & 1.5\% \\
\\[-2ex]
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\captionsetup{font={scriptsize}}
\caption{Semantic Categorization of MovieChat-1K Questions}
\label{tab:q_type}
\end{table}

==> tab/short.tex <==
% \begin{table}[t]
% \centering
% \Large
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{} l c c c c c c @{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{MSVD-QA}} & \multicolumn{2}{c}{\textbf{MSRVTT-QA}} & \multicolumn{2}{c}{\textbf{ActivityNet-QA}} \\
% \cline{2-7}
%  & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score}\\
% \midrule
% FrozenBiLM~\cite{yang2022zero} & 32.2 & -- & 16.8 & -- & 24.7 & -- \\
% Video Chat~\cite{li2023videochat} & 56.3 & 2.8 & 45.0 & 2.5 & 26.5 & 2.2 \\
% LLaMA Adapter~\cite{zhang2023llama} & 54.9 & 3.1 & 43.8 & \underline{2.7} & 34.2 & 2.7 \\
% Video LLaMA~\cite{zhang2023video} & 51.6 & 2.5 & 29.6 & 1.8 & 12.4 & 1.1 \\
% Video-ChatGPT~\cite{maaz2023video} & \underline{64.9} & \underline{3.3} & \underline{49.3} & \textbf{2.8} & \underline{35.2} & \underline{2.7} \\ 
% \midrule
% MovieChat~\textit{(Ours)} & \textbf{75.2} & \textbf{3.8} &\textbf{52.7} & 2.6 & \textbf{45.7} & \textbf{3.4}\\
% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative evaluation for short video question answering with GPT. MovieChat achieves comparable performance even it is not specifically designed for for short video question-answering tasks. The best result is highlighted in bold, and the second best is underlined. The best result is highlighted in bold, and the second best is underlined.}
% \label{tab:short}
% \end{table}


\begin{table}[t]
\centering
\Large
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{MSVD-QA}} & \multicolumn{2}{c}{\textbf{MSRVTT-QA}} & \multicolumn{2}{c}{\textbf{ActivityNet-QA}} \\
\cline{2-7}
 & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score} & \textbf{Accuracy} & \textbf{Score}\\
\midrule
FrozenBiLM~\cite{yang2022zero} & 32.2 & -- & 16.8 & -- & 24.7 & -- \\
Video Chat~\cite{li2023videochat} & 56.3 & 2.8 & 45.0 & 2.5 & 26.5 & 2.2 \\
LLaMA Adapter~\cite{zhang2023llama} & 54.9 & 3.1 & 43.8 & \underline{2.7} & 34.2 & 2.7 \\
Video LLaMA~\cite{zhang2023video} & 51.6 & 2.5 & 29.6 & 1.8 & 12.4 & 1.1 \\
Video-ChatGPT~\cite{maaz2023video} & \underline{64.9} & \underline{3.3} & \underline{49.3} & \textbf{2.8} & \underline{35.2} & \underline{2.7} \\ 
\midrule
MovieChat~\textit{(Ours)} & \textbf{75.2} & \textbf{3.8} &\textbf{52.7} & 2.6 & \textbf{45.7} & \textbf{3.4}\\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for short video question answering with GPT-3.5~\cite{gpt3.5}. MovieChat achieves comparable performance even it is not specifically designed for for short video question-answering tasks. The best result is highlighted in bold, and the second best is underlined. }
\label{tab:short}
\end{table}

==> tab/short_varies.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.61}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
 \scriptsize Video Chat~\cite{li2023videochat} &  \scriptsize 2.23& \scriptsize 2.50& \scriptsize 2.53& \scriptsize 1.94& \scriptsize 2.24\\
 \scriptsize LLaMA Adapter~\cite{zhang2023llama}& \scriptsize 2.03& \scriptsize 2.32& \scriptsize 2.30& \scriptsize 1.98& \scriptsize 2.15\\
 \scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize 1.96& \scriptsize 2.18& \scriptsize 2.16& \scriptsize 1.82& \scriptsize 1.79\\
 \scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize \underline{2.40}& \scriptsize \underline{2.52}& \scriptsize \underline{2.62}& \scriptsize \underline{1.98}& \scriptsize \underline{2.37}\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize \textbf{2.76}& \scriptsize \textbf{2.93}& \scriptsize \textbf{3.01}& \scriptsize \textbf{2.24}& \scriptsize \textbf{2.42} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation for short video generation performance with GPT-3.5~\cite{gpt3.5}. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is highlighted in bold, and the second best is underlined.}
\label{tab:short_varies}
\end{table}

==> tab/videollama_5.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c c c c c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Global Mode}} & \multicolumn{5}{c}{\textbf{Breakpoint Mode}} \\
\cline{2-11}
& \textbf{CI} & \textbf{DO} & \textbf{CU} & \textbf{TU} & \textbf{CO} & \textbf{CI} & \textbf{DO} & \textbf{CU} & \textbf{TU} & \textbf{CO}\\
\midrule
w/o MM &  3.30&  2.53&  3.28&  2.77& 3.42& 2.42& 2.85& 2.87& 2.00& 2.87 \\
base&  \textbf{3.32}&  \textbf{3.28}&  \textbf{3.40}&  \textbf{2.97}& \textbf{3.48}& \textbf{2.97}& \textbf{3.24}& \textbf{3.31}& \textbf{2.70}& \textbf{3.45}\\
\bottomrule
\end{tabular}
}
\caption{Ablation study on how memory mechanism (MM) affects the long video generative performance. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is in bold.}
\label{tab:videollama_5}
\vspace{-5pt}
\end{table}




==> tab/videollama_score.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} c c c c c @{}}
\toprule
\multirow{2}{*}{\textbf{\scriptsize Method}} & \multicolumn{2}{c}{\textbf{\scriptsize Global Mode}} & \multicolumn{2}{c}{\textbf{\scriptsize Breakpoint Mode}} \\
\cline{2-5}
 & \scriptsize {Accuracy} & \scriptsize {Score} & \scriptsize {Accuracy} &  \scriptsize {Score}\\
\midrule
 \rule{0pt}{5pt} \scriptsize w/o MM &   \scriptsize 51.4&  \scriptsize 3.10&  \scriptsize 38.2&  \scriptsize 2.31 \\
  \rule{0pt}{5pt} \scriptsize base&  \scriptsize \textbf{67.8}&  \scriptsize \textbf{3.81}&  \scriptsize \textbf{50.4}& \scriptsize \textbf{2.96} \\
\bottomrule
\end{tabular}
}
\caption{Ablation study on how memory mechanism (MM) affects the long video question answering. The best result is in bold.}
\label{tab:videollama_score}
\vspace{-5pt}
\end{table}



==> tab_tpami/ego_various.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.61}
\caption{Quantitative evaluation for long video generation performance with the average of GPT-3.5~\cite{gpt3.5}, Claude~\cite{examplewebpage} and human blind rating. CI stands for correctness of information, DO stands for detail orientation, CU stands for contextual understanding, TU stands for temporal understanding, and CO stands for consistency. The best result is in bold, and the second best is underlined.}
\label{tab_tpami:ego_varies}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{Text Decoder} & \scriptsize \textbf{CI} & \scriptsize \textbf{DO} & \scriptsize \textbf{CU} & \scriptsize \textbf{TU} & \scriptsize \textbf{CO}\\
\midrule
GIT~\cite{wang2022git} & \scriptsize non-LLM based & -- & -- & -- & -- & -- \\
mPLUG-2~\cite{xu2023mplug} & \scriptsize non-LLM based &  -- & -- & -- & -- & -- \\
FrozenBiLM~\cite{yang2022zero} & \scriptsize non-LLM based & -- & -- & -- & -- & -- \\
\midrule
\scriptsize Video Chat~\cite{li2023videochat} & \scriptsize LLM based &-- & -- & -- & -- & --\\
\scriptsize Video LLaMA~\cite{zhang2023video} & \scriptsize LLM based & -- & -- & -- & -- & --\\
\scriptsize Video-ChatGPT~\cite{maaz2023video}& \scriptsize LLM based & -- & -- & -- & -- & --\\
\midrule
\scriptsize MovieChat~\textit{(Ours)}& \scriptsize LLM based & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
}

\end{table}

==> tab_tpami/short_2.tex <==
\begin{table}[t]
\centering
\Large
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.3}
\caption{Quantitative evaluation for short video question answering with GPT-3.5~\cite{gpt3.5}. MovieChat achieves comparable performance even it is not specifically designed for for short video question-answering tasks. The best result is highlighted in bold, and the second best is underlined. Acc. and Sco. stand for accuracy and score respectively.}
\label{tab_tpami:short}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c c c c c @{}}
\toprule
\multirow{1}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{MSVD-QA}} & \multicolumn{2}{c}{\textbf{MSRVTT-QA}} & \multicolumn{2}{c}{\textbf{ActivityNet-QA}} \\
\cline{2-7}
 & \textbf{Acc.} & \textbf{Sco.} & \textbf{Acc.} & \textbf{Sco.} & \textbf{Acc.} & \textbf{Sco.}\\
\midrule
FrozenBiLM~\cite{yang2022zero} & 2.2 & -- & 16.8 & -- & 24.7 & -- \\
\midrule
Video Chat~\cite{li2023videochat} & 56.3 & 2.8 & 45.0 & 2.5 & 26.5 & 2.2 \\
LLaMA Adapter~\cite{zhang2023llama} & 54.9 & 3.1 & 43.8 & \underline{2.7} & 34.2 & \underline{2.7} \\
Video LLaMA~\cite{zhang2023video} & 51.6 & 2.5 & 29.6 & 1.8 & 12.4 & 1.1 \\
Video-ChatGPT~\cite{maaz2023video} & 64.9 & 3.3 & 49.3 & \textbf{2.8} & 35.2 & \underline{2.7} \\ 
\midrule
MovieChat & \underline{75.2} & \underline{3.8} &\underline{52.7} & 2.6 & \underline{45.7} & \textbf{3.4}\\
MovieChat+ & \textbf{76.5} & \textbf{3.9} &\textbf{52.9} & \underline{2.7} & \textbf{47.1} & \textbf{3.4}\\
\bottomrule
\end{tabular}
}

\end{table}

==> tab_tpami/tem_agg.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.7}
\caption{Comparisons between pre- and post-LLM temporal context aggregation. Acc. stands for accuracy based on EgoSchema~\cite{mangalam2023egoschema}}
\label{tab_tpami:tem_agg}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l c c @{}}
\toprule
\scriptsize \textbf{Method} & \scriptsize \textbf{Aggregate pre-LLM} & \scriptsize \textbf{Acc.} \\
\midrule
\scriptsize Base & \scriptsize \times & \scriptsize33.25 \\
\scriptsize Base & \scriptsize \checkmark & \scriptsize33.39 \\
 \\[-1.5ex]
\midrule
 \\[-1.5ex]
\scriptsize Memory Consolidation (Ours) & \scriptsize \checkmark & \scriptsize34.62 \\

\bottomrule
\end{tabular}
}
\end{table}
